Promptable Game Models: Text-Guided Game Simulation via Masked Diffusion Models

Neural video game simulators emerged as powerful tools to generate and edit videos. Their idea is to represent games as the evolution of an environment's state driven by the actions of its agents. While such a paradigm enables users to play a game action-by-action, its rigidity precludes more semantic forms of control. To overcome this limitation, we augment game models with prompts specified as a set of natural language actions and desired states. The result-a Promptable Game Model (PGM)-makes it possible for a user to play the game by prompting it with high- and low-level action sequences. Most captivatingly, our PGM unlocks the director's mode, where the game is played by specifying goals for the agents in the form of a prompt. This requires learning "game AI", encapsulated by our animation model, to navigate the scene using high-level constraints, play against an adversary, and devise a strategy to win a point. To render the resulting state, we use a compositional NeRF representation encapsulated in our synthesis model. To foster future research, we present newly collected, annotated and calibrated Tennis and Minecraft datasets. Our method significantly outperforms existing neural video game simulators in terms of rendering quality and unlocks applications beyond the capabilities of the current state of the art. Our framework, data, and models are available at https://snap-research.github.io/promptable-game-models/.

==> tables/table_dataset_caption_statistics.tex <==

\begin{table}[t]
\caption{Dataset caption statistics for the Tennis and Minecraft datasets.}

\label{table:dataset_caption_statistics}

\begin{center}

%\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lcc}
\toprule
 & Tennis  & Minecraft \\
\midrule

Captions & 84.1k & 818k \\
\;\;\;\emph{of which unique} & 25.5k & 1.24k \\
Unique words & 915 & 117 \\
Avg. words & 13.8 & 5.85 \\
Avg. span & 1.32s & 0.500s \\

\bottomrule
\end{tabular}
\end{center}

\end{table}


==> tables/table_dataset_video_statistics.tex <==

\begin{table}[t]
\caption{Dataset statistics for the Tennis and Minecraft datasets.}

\label{table:dataset_video_statistics}

\begin{center}

%\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lcc}
\toprule
 & Tennis  & Minecraft \\
\midrule

Sequences: & 7112 & 61 \\
\;\;\;\emph{train} & 5690 & 51 \\
\;\;\;\emph{validation} & 711 & 5 \\
\;\;\;\emph{test} & 711 & 5 \\
\midrule
Duration: & 15.5h & 1.21h \\
\;\;\;\emph{train} & 12.4h & 0.952h \\
\;\;\;\emph{validation} & 1.59h & 0.16h \\
\;\;\;\emph{test} & 1.52h & 0.101 \\
\midrule
Annotated frames: & 9.70M & 599k \\
\;\;\;\emph{train} & 9.44M & 581k \\
\;\;\;\emph{validation} & 135k & 11.2k \\
\;\;\;\emph{test} & 130k & 7.06k \\
\midrule
Resolution & 1920x1080px & 1024x576px \\
Framerate & 25fps & 20fps \\

\bottomrule
\end{tabular}
\end{center}

\end{table}



==> tables/table_synthesis_minecraft.tex <==

\begin{table}[t]

\caption{Comparison with baselines and ablation on the Minecraft dataset. MDR in \%, ADD in pixels. $\dag$ denotes output in 512x288px rather than 1024x576px resolution.}

\label{table:synthesis_minecraft}

\begin{center}

%\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lccccc}
\toprule
 & LPIPS$\downarrow$  & FID$\downarrow$ & FVD$\downarrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule

PE$^\dag$ \cite{Menapace2022PlayableEnvironments} & \cellthird0.0235 & \cellthird13.9 & \cellthird21.5 & \cellthird5.77 & \cellthird0.0412  \\
PE+ \cite{Menapace2022PlayableEnvironments} & 0.0238 & 15.5 & 51.7 & 120.6 & 0.939  \\
\midrule
Ours Small & \cellsecond0.00996 & \cellsecond3.56 & \cellsecond8.83 & \cellsecond2.02 & \cellsecond0.0529  \\
Ours & \cellfirst0.00814 & \cellfirst2.81 & \cellfirst7.08 & \cellfirst1.98 & \cellfirst0.0508  \\

\bottomrule
\end{tabular}
\end{center}

\end{table}

==> tables/table_synthesis_tennis.tex <==

\begin{table}[t]
\caption{Comparison with baselines and ablation on the Tennis dataset. MDR in \%, ADD in pixels. Note that FID and FVD are computed on images downscaled to the feature extractor training resolution, thus blurriness in the PE baseline caused by its reduced resolution is not captured by these metrics. LPIPS correctly reflects lack of sharpness in the PE results (see Fig.~\ref{fig:synthesis_ablation_qualitatives}). $\dag$ denotes output in 512x288px rather than 1024x576px resolution.}

\label{table:synthesis_tennis}

\begin{center}

%\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lccccc}
\toprule
 & LPIPS$\downarrow$  & FID$\downarrow$ & FVD$\downarrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule

PE$^\dag$ \cite{Menapace2022PlayableEnvironments} & 0.188 & \cellfirst11.5 & \cellfirst349 & 3.74 & 0.200  \\
PE+ \cite{Menapace2022PlayableEnvironments} & 0.232 & 40.4 & 2432 & 132.3 & 49.7  \\
\midrule
w/o enhancer $\netenhancer$ & \cellthird0.167 & 15.6 & 570 & \cellthird3.02 & 0.0728  \\
w/o explicit deformation in $\netdeformation$ & \cellsecond0.156 & 13.3 & 524 & 3.10 & 0.0587  \\
w/o planes in $\netcanonical$ & 0.241 & 30.4 & 1064 & \cellsecond2.94 & 0.0611  \\
w/o voxels in $\netcanonical$ & 0.170 & 17.1 & 757 & 3.03 & \cellfirst0.0399  \\
w/o our encoder $\netstyle$ & 0.174 & 15.0 & 600 & 3.18 & 0.0564  \\
\midrule
Ours Small & \cellsecond0.156 & \cellthird13.4 & \cellthird523 & \cellfirst2.88 & \cellthird0.0470  \\
Ours & \cellfirst0.152 & \cellsecond12.8 & \cellsecond516 & \cellfirst2.88 & \cellsecond0.0423  \\

\bottomrule
\end{tabular}
\end{center}

\end{table}
